Multi-Fidelity Bayesian Optimisation of Wind Farm Wake Steering using Wake Models and Large Eddy Simulations

Improving the power output from wind farms is vital in transitioning to renewable electricity generation. However, in wind farms, wind turbines often operate in the wake of other turbines, leading to a reduction in the wind speed and the resulting power output whilst also increasing fatigue. By using wake steering strategies to control the wake behind each turbine, the total wind farm power output can be increased. To find optimal yaw configurations, typically analytical wake models have been utilised to model the interactions between the wind turbines through the flow field. In this work we show that, for full wind farms, higher-fidelity computational fluid dynamics simulations, in the form of large eddy simulations, are able to find more optimal yaw configurations than analytical wake models. This is because they capture and exploit more of the physics involved in the interactions between the multiple turbine wakes and the atmospheric boundary layer. As large eddy simulations are much more expensive to run than analytical wake models, a multi-fidelity Bayesian optimisation framework is introduced. This implements a multi-fidelity surrogate model, that is able to capture the non-linear relationship between the analytical wake models and the large eddy simulations, and a multi-fidelity acquisition function to determine the configuration and fidelity of each optimisation iteration. This allows for fewer configurations to be evaluated with the more expensive large eddy simulations than a single-fidelity optimisation, whilst producing comparable optimisation results. The same total wind farm power improvements can then be found for a reduced computational cost.

==> Makefile <==
NAME = Paper
BUILDDIR = build
PDFLATEX = max_print_line=1048576 pdflatex -file-line-error \
           -halt-on-error --shell-escape --output-directory=$(BUILDDIR)
PDFLATEXSTD = pdflatex -halt-on-error
TEXFILE = $(NAME).tex
TEXPDFFILES = $(BUILDDIR)/${TEXFILE:.tex=.pdf}
SECTIONFILES = $(shell find Sections -name '*.tex' -print)
BIBFILES = *.bib
STYFILES = sn-jnl.cls
BSTFILES = bst/*

rwildcard=$(foreach d,$(wildcard $(1:=/*)),$(call rwildcard,$d,$2) $(filter $(subst *,%,$2),$d))

SVGFILES := $(call rwildcard,./Sections,*.svg)
SVGPDFFILES = ${SVGFILES:.svg=.pdf}
INKSCAPE = inkscape

$(TEXPDFFILES): $(BUILDDIR)/%.pdf: %.tex $(BIBFILES) $(SVGPDFFILES) $(SECTIONFILES) $(STYFILES) $(BSTFILES)
	$(PDFLATEX) $(@F:.pdf=)
	cp $(BIBFILES) $(BUILDDIR)
	cp $(STYFILES) $(BUILDDIR)
	cp $(BSTFILES) $(BUILDDIR)
	cd $(BUILDDIR) && bibtex $(@F:.pdf=)
	$(PDFLATEX) $(@F:.pdf=)
	$(PDFLATEX) $(@F:.pdf=)

%.pdf : %.svg
	$(INKSCAPE) -A $*.pdf $*.svg

clean:
	rm -rf $(BUILDDIR)/*
	rm -f $(SVGPDFFILES)

# Ensure build directory is created before output files
$(TEXPDFFILES): | dirs
.PHONY: dirs
dirs:
	mkdir -p build


